Flash-SD-KDE: Accelerating SD-KDE with Tensor Cores

Score-debiased kernel density estimation (SD-KDE) achieves improved asymptotic convergence rates over classical KDE, but its use of an empirical score has made it significantly slower in practice. We show that by re-ordering the SD-KDE computation to expose matrix-multiplication structure, Tensor Cores can be used to accelerate the GPU implementation. On a 32k-sample 16-dimensional problem, our approach runs up to $47\times$ faster than a strong SD-KDE GPU baseline and $3{,}300\times$ faster than scikit-learn's KDE. On a larger 1M-sample 16-dimensional task evaluated on 131k queries, Flash-SD-KDE completes in $2.3$ s on a single GPU, making score-debiased density estimation practical at previously infeasible scales.

==> sections/07_impact.tex <==
\section*{Impact Statement}

This paper presents work whose goal is to accelerate SD-KDE and KDE kernels on
GPUs. We expect the primary impact to be enabling practitioners to apply these
estimators to larger datasets; we do not foresee unique societal consequences
outside the usual considerations for density estimation applications.

